DARE: A large-scale handwritten date recognition system

Handwritten text recognition for historical documents is an important task but it remains difficult due to a lack of sufficient training data in combination with a large variability of writing styles and degradation of historical documents. While recurrent neural network architectures are commonly used for handwritten text recognition, they are often computationally expensive to train and the benefit of recurrence drastically differs by task. For these reasons, it is important to consider non-recurrent architectures. In the context of handwritten date recognition, we propose an architecture based on the EfficientNetV2 class of models that is fast to train, robust to parameter choices, and accurately transcribes handwritten dates from a number of sources. For training, we introduce a database containing almost 10 million tokens, originating from more than 2.2 million handwritten dates which are segmented from different historical documents. As dates are some of the most common information on historical documents, and with historical archives containing millions of such documents, the efficient and automatic transcription of dates has the potential to lead to significant cost-savings over manual transcription. We show that training on handwritten text with high variability in writing styles result in robust models for general handwritten text recognition and that transfer learning from the DARE system increases transcription accuracy substantially, allowing one to obtain high accuracy even when using a relatively small training sample.

==> tex/old-result-tables.tex <==
% \begin{table*}[!ht]
% \centering
% \begin{threeparttable}[b]
% \begin{center}
% \scriptsize
% \caption{Performance Results of \co{name models above and put here}}
% \label{tab:individual}
% \centering
% \begin{tabular}{lcccc}
% \thickhline
%  \textbf{Dataset} & \textbf{Sequence} & \textbf{SeqAcc} & \textbf{SeqAcc@90} \\
% \thickhline
%  \textbf{DC-1} & DD-M-YYYY & {97.30}\% & {98.44}\% \\
%   \thickhline
%  \textbf{DC-2} & DD-M-YYYY & {92.78}\% & {98.25}\% \\
%   \thickhline
%  \textbf{PR-1} & DD-M-YY & {93.47}\% & {96.18}\% \\
%   \thickhline
%  \textbf{PR-2} & DD-M-YY & 81.49\% & 87.54\% \\
%   \thickhline
%  \textbf{SWE-BD} & DD-M-YY & 94.58\% & {97.84}\%  \\
%   \thickhline
%  \textbf{FR} & DD-M & \textbf{98.24}\% & {98.92}\%  \\
%   \thickhline
%  \textbf{NHVD}  & DD-M & \textbf{97.53}\% & {98.67}\%\\
%   \thickhline
%  \textbf{SWE-DD} & DD-M & {99.39}\% & {99.79}\% \\
% \thickhline
% \thickhline
% \end{tabular}
% \begin{tablenotes}[flushleft]
%       \item{\scriptsize{The table shows the test performance of the models as measured by SeqAcc, where each row represents a unique model trained only on that dataset (indicated by thick lines between models).
%       SeqAcc@90 is the SeqAcc when we remove the 10\% of test predictions where the model is the most uncertain about its prediction.¨
%       \co{TODO once with names, add column with name of model}
%       }}
%     \end{tablenotes}
% \end{center}
% \end{threeparttable}
% \end{table*}

% \begin{table*}[!ht]
% \centering
% \begin{threeparttable}[b]
% \begin{center}
% \scriptsize
% \caption{Performance Results of \co{name model above and put here}}
% \label{tab:combined1}
% \centering
% \begin{tabular}{lcccc}
% \thickhline
%  \textbf{Dataset} & \textbf{Sequence} & \textbf{SeqAcc} & \textbf{SeqAcc@90} \\
% \thickhline
%  \textbf{DC-1} & DD-M-YYYY & 96.70\% & 98.33\%\\
%  \textbf{DC-2} & DD-M-YYYY & 91.59\% &  98.61\% \\
%  \textbf{PR-1} & DD-M-YY & 94.00\% & 96.72\%  \\
%  \textbf{PR-2} & DD-M-YY &  82.71\% & 88.86\% \\
%  \textbf{SWE-BD} & DD-M-YY & 94.75\% & 98.42\% \\
%  \textbf{FR} & DD-M & 98.19\% & 99.25\% \\
%  \textbf{NHVD}  & DD-M & 97.48\% & 98.15\% \\
%  \textbf{SWE-DD} & DD-M & 99.35\% & \textbf{99.90}\% \\
%   \thickhline
% \thickhline
% \end{tabular}
% \begin{tablenotes}[flushleft]
%       \item{\scriptsize{The table shows the test performance of the model trained on all datasets as measured by SeqAcc. 
%       SeqAcc@90 is the SeqAcc when we remove the 10\% of test predictions where the model is the most uncertain about its prediction.
%       While trained jointly on all datasets, we report test performance separately for each test set, to see how the performance differs between datasets
%     %   Note that even though some date sequences might be longer on the images than on their corresponding labels, this is not included if the labels do not consistently reflect this.
%     %   All data sources are restricted to the maximum of the date sequence while remaining consistent, as discussed in Section~\ref{sec: Constructing the DARE Database}.
%       }}
%     \end{tablenotes}
% \end{center}
% \end{threeparttable}
% \end{table*}


% \begin{table*}[!ht]
% \centering
% \begin{threeparttable}[b]
% \begin{center}
% \scriptsize
% \caption{Performance Results of \co{name models above and put here}}
% \label{tab:combined2}
% \centering
% \begin{tabular}{lcccc}
% \thickhline
%  \textbf{Dataset} & \textbf{Sequence} & \textbf{SeqAcc} & \textbf{SeqAcc@90} \\
% \thickhline
%  \textbf{DC-1} & DD-M-YY &  {\textbf{98.30}}\% & {\textbf{98.67}}\%\\
%  \textbf{DC-2} & DD-M-YY &  \underline{\textbf{97.19}}\% &  \underline{\textbf{99.28}}\% \\
%  \textbf{PR-1} & DD-M-YY & \textbf{95.97}\%  &  \textbf{97.90}\% \\
%  \textbf{PR-2} & DD-M-YY &  \textbf{84.79}\% & \textbf{90.60}\% \\
%  \textbf{SWE-BD} & DD-M-YY & \textbf{96.29}\% & \textbf{98.78}\% \\
% \thickhline
%  \textbf{FR} & DD-M & \textbf{98.24}\% & \textbf{99.14}\% \\
%  \textbf{NHVD}  & DD-M  & 97.52\% & \textbf{98.69}\% \\ 
%   \textbf{SWE-DD} & DD-M & \textbf{99.40}\% & {99.83}\%  \\
% \thickhline
% \thickhline
% \end{tabular}
% \begin{tablenotes}[flushleft]
%       \item{\scriptsize{The table shows the test performance of the two models trained on separate subsets of the DARE database, as measured by SeqAcc.
%       Above the thick line, \co{model X, below model Y, name!}.
%       SeqAcc@90 is the SeqAcc when we remove the 10\% of test predictions where the model is the most uncertain about its prediction.
%     %   The models are trained on two subsets of aggregated training datasets.
%     %   Model 1 is trained on the day, month, and year and tested on the individual test datasets of these five combined datasets.
%     %   Model 2 is trained on the day and month, as the three used datasets only contain this information reliably, as discussed in Section~\ref{sec: Constructing the DARE Database}. 
%     %   Note that the sequence length for death certificates is shorter in this table relative to Tables~\ref{tab:individual} and \ref{tab:combined1}, as we exclude the century label in this model.
%     }}
%     \end{tablenotes}
% \end{center}
% \end{threeparttable}
% \end{table*}




\FloatBarrier
\newpage

 \section{Details on Data Sources}
\label{sec: Details on Data Sources}
In this appendix, we provide additional visualizations on the datasets we use to construct the DARE database.

\section{Additional Linking Details}
This section provides additional details on our linking procedure discussed in Section \ref{sec: linking}. The pipeline that we use for linking the 1916 Danish census is visualized in Figure \ref{fig:linking_expanded}. The figure starts from the initial prediction obtained directly from the DARE system and the name models from \citet{dahl2022hana}. This roughly corresponds to 8,000 predictions which are obtained primarily from matching based on the first name in combination with the date and the first and last name. By sample splitting we use half of these matched predictions to train models 1.1 (which consists of three models) and the other half to train models 2.1 (which also consists of three models). We find that this very small training sample vastly increases the matches we are able obtain in round 1. Here, we use the intersection between the matches obtained from models 1.1 and models 2.1 and find that the intersection of the matches now increase with more than 100,000. Also, it seems important that more predictions are now matched using the ``all'' criteria, implying that the model and the manually transcription are in agreement on both the date, first name, and last name. The 50\% sample split is introduced in order to avoid overfitting on our data and thereby holding onto poorly linked transcription. After tuning the network, we once again predict the full
census records and perform the same linking procedure as described above with. We continue to do so until only a small amount of additional linked entries are obtained. Going from round 3 to 4 we only obtain an additional 576 matched entries. From the 143,044 matched entries we train a final model which uses the full matched dataset from which we extract our final transcriptions achieving an approximate 90-95\% date accuracy % (based on Table \ref{tab: transcription-census}) 
on the entire 3.7 million entries in the 1916 Danish census.

%\newgeometry{left=2.5cm,right=2.5cm,top=1.5cm,bottom=2.5cm}

\begin{center}
    \begin{figure*}
    
        % \captionsetup{width=1\linewidth}
        \caption{Predictions Linked to the Danish Census: 4 Identifiers with Sample Splitting}
        \label{fig:linking_expanded}
        \centering
        \scriptsize{
        \begin{tikzpicture}[scale=1.4]
        %  \draw[dotted](-0.5,0.5) -- (2.5,0.5);
        %  \draw[dotted](2.5,0.5) -- (2.5,2.5) ;
        %   \draw[dotted](2.5,0.5) -- (2.5,2.5);
        %  \draw[dotted](-0.5,0.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 0}}} ;
        %  \draw[dotted](0.5,1.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 1}}} ;
        %  \draw[dotted](1.5,2.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 2}}} ;
        % \draw[dotted](2.5,3.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 3}}} ;
        % \draw[dotted](3.5,4.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 4}}} ; \draw[dotted](4.5,5.5) -- (0,0) node [midway, left] {\Large\textbf{{Round 5}}} ;
        %  \draw node  to [out=330,in=300,looseness=8] (3);
        %  \draw[dotted](2.5,2.5) -- (-0.5,2.5);
        %  \draw[dotted](-0.5,2.5) -- (-0.5,0.5);
        
        %    \GraphInit[vstyle=Classic]
        \SetUpVertex[Lpos=-90]
        %      \tikzset{VertexStyle/.style = {shape=ellipse, fill=black,
        %                           minimum size=13pt,inner sep=0pt}
        %      }
        
        \SetGraphUnit{3} 
        
        % Rows
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round0) at (0,8.5) {\textbf{Round 0}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round1) at (0,6.5) {\textbf{Round 1}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round2) at (0,4.5) {\textbf{Round 2}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round3) at (0,2.5) {\textbf{Round 3}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round4) at (0,0.5) {\textbf{Round 4}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Round5) at (0,-1.5) {\textbf{Round 5}};
        
        % Columns
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Model1) at (2.2,9.6) {\textbf{Model 1}};
        
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (All) at (1,9.2) {\textbf{All}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Lastname and date) at (1.8,9) {\textbf{First \& date}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Firstname and date) at (2.6,9.2) {\textbf{Last \& date}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Firstname and lastname) at (3.4,9) {\textbf{First \& last}};
        
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Model2) at (6.8,9.6) {\textbf{Model 2}};
        
        
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (All2) at (5.6,9.2) {\textbf{All}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Lastname and date2) at (6.4,9) {\textbf{First \& date}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Firstname and date2) at (7.2,9.2) {\textbf{Last \& date}};
        \node[circle,text=black, fill =lightgray,text opacity = 1,fill opacity=0.00] (Firstname and lastname2) at (8,9) {\textbf{First \& last}};
        
        % Round 5
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (5) at (2.2,-1) {Models 1.5};
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (Final5) at (6.8,-1) {Final transcriptions};
        
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (511) at (1,-1.5) {134,367};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (512) at (1.8,-1.5) {6,013};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (513) at (2.6,-1.5) {4,649};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (514) at (3.4,-1.5) {1,052};
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (53) at (5,-1.5) {146,081};
        
        % Round 4
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (411) at (1,0.5) {122,405};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (412) at (1.8,0.5) {8,922};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (413) at (2.6,0.5) {6,626};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (414) at (3.4,0.5) {7,111};
        
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (421) at (5.6,0.5) {122,307};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (422) at (6.4,0.5) {8,923};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (423) at (7.2,0.5) {6,664};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (424) at (8,0.5) {7,156};
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (43) at (4.5,-0.5) {$\cap$ 143,044};
        
        % Round 3
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (311) at (1,2.5) {120,118};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (312) at (1.8,2.5) {10,350};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (313) at (2.6,2.5) {7,011};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (314) at (3.4,2.5) {7,132};
        
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (321) at (5.6,2.5) {120,915};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (322) at (6.4,2.5) {9,501};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (323) at (7.2,2.5) {7,016};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (324) at (8,2.5) {7,360};
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (33) at (4.5,1.5) {$\cap$ 142,468};
        
        % Round 2
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (211) at (1,4.5) {114,424};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (212) at (1.8,4.5) {11,077};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (213) at (2.6,4.5) {8,272};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (214) at (3.4,4.5) {9,713};
        
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (221) at (5.6,4.5) {114,797};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (222) at (6.4,4.5) {10,864};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (223) at (7.2,4.5) {8,129};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (224) at (8,4.5) {9,714};
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (23) at (4.5,3.5) {$\cap$ 140,674};
        
        % Round 1
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (111) at (1,6.5) {67,688};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (112) at (1.8,6.5) {17,867};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (113) at (2.6,6.5) {17,982};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (114) at (3.4,6.5) {16,175};
        
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (121) at (5.6,6.5) {69,874};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (122) at (6.4,6.5) {18,954};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (123) at (7.2,6.5) {17,581};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (124) at (8,6.5) {15,282};
        
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (13) at (4.5,5.5) {$\cap$ 108,353};
        
        
        % Round 0
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (011) at (1,8.5) {816};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (012) at (1.8,8.5) {4,538};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (013) at (2.6,8.5) {405};
        \node[ellipse,text=black, fill =brown,text opacity = 1,fill opacity=0.1] (014) at (3.4,8.5) {2,186};
        
        \node[ellipse,text=black, fill =cyan,text opacity = 1,fill opacity=0.1] (03) at (4.5,7.5) {7,945};
        
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M11) at (2.2,7) {Models 1.1};
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M21) at (6.8,7) {Models 2.1};
        
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M12) at (2.2,5) {Models 1.2};
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M22) at (6.8,5) {Models 2.2};
        
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M13) at (2.2,3) {Models 1.3};
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M23) at (6.8,3) {Models 2.3};
        
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M14) at (2.2,1) {Models 1.4};
        \node[ellipse,text=black, fill =teal,text opacity = 1,fill opacity=0.1] (M24) at (6.8,1) {Models 2.4};
        
        
        
        \tikzset{EdgeStyle/.style={->,font=\scriptsize},{below=15pt}}
        \foreach \j in {1,...,4}{\foreach \i in {1,...,1}{\Edge[](01\j)(03)}}
        
        
        \foreach \m in {1,...,4} \foreach \j in {1,...,4}
        {\foreach \i in {1,...,2}{\Edge[](\m\i\j)(\m3)}}
        
        \foreach \i in {1,...,4}{\Edge[](M11)(11\i)}
        \foreach \i in {1,...,4}{\Edge[](M21)(12\i)}
        
        \foreach \i in {1,...,4}{\Edge[](M12)(21\i)}
        \foreach \i in {1,...,4}{\Edge[](M22)(22\i)}
        
        \foreach \i in {1,...,4}{\Edge[](M13)(31\i)}
        \foreach \i in {1,...,4}{\Edge[](M23)(32\i)}
        
        \foreach \i in {1,...,4}{\Edge[](M14)(41\i)}
        \foreach \i in {1,...,4}{\Edge[](M24)(42\i)}
        
        \foreach \i in {1,...,4}{\Edge[](5)(51\i)}
        
        \draw[->,ultra thick] (03) to node[above,sloped] {50\%} (M11);
        \draw[->,ultra thick] (03) to node[above,sloped] {50\%} (M21);
        
        \draw[->,ultra thick] (13) to node[above,sloped] {50\%} (M12);
        \draw[->,ultra thick] (13) to node[above,sloped] {50\%} (M22);
        
        \draw[->,ultra thick] (23) to node[above,sloped] {50\%} (M13);
        \draw[->,ultra thick] (23) to node[above,sloped] {50\%} (M23);
        
        \draw[->,ultra thick] (33) to node[above,sloped] {50\%} (M14);
        \draw[->,ultra thick] (33) to node[above,sloped] {50\%} (M24);
        
        \draw[->,ultra thick] (43) to node[above,sloped] {100\%} (5);
        \tikzset{EdgeStyle/.style={->,font=\scriptsize},{below=15pt}}
        
        \Edge[](514)(53)
        \Edge[](5)(Final5)
        \end{tikzpicture}}
        \begin{minipage}{1\linewidth}
        \linespread{1.0}\selectfont
            \vspace{1ex}
            \footnotesize{
            \textit{Notes:}
            This figure visualize the process for linking the predictions to the manually transcribed census records. Initially in round 0 we predict on the full census data from 1916. From these predictions we are able to initially link almost 8k transcriptions to the manual records. We combine matches obtained from using any of the possible unique person identifiers in pairs of at least two exact identifiers being equal to the manual records. As we gradually remove instances from the manually transcribed census records, we also obtain a smaller matching data for linking the predictions. Hence, we can repeat the process of exactly matching as the number of obtainable matches gradually decrease as we alternate between these three personal identifiers.  We repeat the linking process until no more matches are obtainable yielding a total of 7,945 matches after round 0.  We can now use the newly found matches for transfer learning (tuning) our network to the Danish census. To avoid overfitting on our data and thereby holding onto poorly linked transcription we use a sample splitting procedure, implying that we train two models at each stage training on only 50\% of the data each. After tuning the network, we predict the full census records and perform the same linking procedure as described above with the only exception being that we only hold onto linked transcriptions that are by both networks linked to the same manual transcript. 
            }
        \end{minipage}
    \end{figure*}
\end{center}


==> tex/param_tab.tex <==
%RandAugment            &  $N=2,M=7$ &       $N=2,M=7$ &                %$N=2,M=7$ &                $N=2,M=7$ &    $N=2,M=7$ \\
%Batch size             &        256 &             308 &                      308 &                      308 &          308 \\
%Gradient clip value    &       0.02 &            0.02 &                     0.02 &                     0.02 &         0.02 \\
%Dropout prob.          &        0.4 &             0.4 &                      0.4 &                      0.4 &          0.4 \\
%Stochastic depth prob. &       0.25 &            0.25 &                     0.25 &                     0.25 &         0.25 \\
%Epochs                 &        240 &             240 &                       90 &                      120 &           60 \\
%Learning rate          &        0.5 &             0.6 &                      0.6 &                      0.6 &          0.6 \\
%Momentum               &        0.9 &             0.9 &                      0.9 &                      0.9 &          0.9 \\
%Random erase prob.     &        0.4 &             0.4 &                      0.4 &                      0.4 &          0.4 \\
%Label smoothing        &        0.1 &             0.1 &                      0.1 &                      0.1 &          0.1 \\
%Weight decay           &   0.000007 &        0.000007 &                 0.000007 &                 0.000007 &     0.000007 \\
%\bottomrule


%RandAugment            &  $N=2,M=7$ &   -    &   -  &     -  &    - \\
%Batch size             &        256 &             308 &                      - &                      - &          - \\
%Gradient clip value    &       0.02 &            - &                     - &                     - &         - \\
%Dropout prob.          &        0.4 &             - &                      - &                      - &          - \\
%Stochastic depth prob. &       0.25 &            - &                     - &                     - &         - \\
%Epochs                 &        240 &             - &                       90 &                      120 &           60 \\
%Learning rate          &        0.5 &             0.6 &                      - &                      - &          - \\
%Momentum               &        0.9 &             - &                      - &                      - &          - \\
%Random erase prob.     &        0.4 &             - &                      - &                      - &          - \\
%Label smoothing        &        0.1 &             - &                      - &                      - &          - \\
%Weight decay           &   0.000007 &        - &                 - &                 - &     - \\
%\bottomrule


